Solving Large-Scale Granular Resource Allocation Problems Efficiently with POP

Resource allocation problems in many computer systems can be formulated as mathematical optimization problems. However, finding exact solutions to these problems using off-the-shelf solvers is often intractable for large problem sizes with tight SLAs, leading system designers to rely on cheap, heuristic algorithms. We observe, however, that many allocation problems are granular: they consist of a large number of clients and resources, each client requests a small fraction of the total number of resources, and clients can interchangeably use different resources. For these problems, we propose an alternative approach that reuses the original optimization problem formulation and leads to better allocations than domain-specific heuristics. Our technique, Partitioned Optimization Problems (POP), randomly splits the problem into smaller problems (with a subset of the clients and resources in the system) and coalesces the resulting sub-allocations into a global allocation for all clients. We provide theoretical and empirical evidence as to why random partitioning works well. In our experiments, POP achieves allocations within 1.5% of the optimal with orders-of-magnitude improvements in runtime compared to existing systems for cluster scheduling, traffic engineering, and load balancing.

==> listing_macros.tex <==
\usepackage{listings}
% we could try "minted" for highlighting

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstdefinestyle{MyCodeStyle}
%\lstset{ %
{
backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=true,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  %deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={!}{!},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  %frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  morekeywords={function,local},            % if you want to add more keywords to the set
  numbers=left,
  numberstyle=\footnotesize\color{mygray},
  xleftmargin=1.8em,
  numbersep=0.8em,
  aboveskip=0pt,
  belowskip=0pt,
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname,                   % show the filename of files included with \lstinputlisting; also try caption instead of title
  basicstyle=\ttfamily,
  columns=flexible
}

\lstset{
language=C,                 % the language of the code
}

\usepackage{silence}
\WarningFilter{latex}{Text page iii contains only floats}


%%%%%%%%%%%%%%%
% listing syntax for ModP
%%%%%%%%%%%%%%%
% Define Language
\lstloadlanguages{[Visual]C++}
\lstdefinelanguage{modp}
{
  % list of keywords
  morekeywords={
    module,
    machine,
    refines,
    satisfies,
    test,
    hide,
    in,
    sends,
    send,
    creates,
    private,
    receives, 
    implementation,
    specification, 
    event, 
    model, 
    \$,
    bool,
    any, 
    static, 
    fun, 
    if, 
    int, 
    interface,
    entry,
    state, 
    var,
    new,
    goto,
    hot,
    start,
    on,
    monitor,
    observes,
    eventset, 
    is
  },
  sensitive=false, % keywords are not case-sensitive
  morecomment=[l]{//}, % l is for line comment
  morecomment=[s]{/*}{*/}, % s is for start and end delimiter
  morestring=[b]" % defines that strings are enclosed in double quotes
}

\definecolor{eclipseBlue}{RGB}{42,0.0,255}
\definecolor{eclipseGreen}{RGB}{0, 139, 69}
\definecolor{eclipsePurple}{RGB}{127,0,85}

\lstdefinestyle{ModPCodeStyle}
{
  basicstyle=\ttfamily\footnotesize, % Global Code Style
  captionpos=b, % Position of the Caption (t for top, b for bottom)
  extendedchars=true, % Allows 256 instead of 128 ASCII characters
  tabsize=2, % number of spaces indented when discovering a tab
  columns=fixed, % make all characters equal width
  keepspaces=true, % does not ignore spaces to fit width, convert tabs to spaces
  showstringspaces=false, % lets spaces in strings appear as real spaces
  breaklines=true, % wrap lines if they don't fit
  numbers=left,
  xleftmargin=1.8em,
  numbersep=0.8em,
  aboveskip=0pt,
  belowskip=0pt,
  %frame=tb, % draw a frame at the top, right, left and bottom of the listing
  %frameround=tttt, % make the frame round at all four corners
  %framesep=4pt, % quarter circle size of the round corners
  %numbers=right, % show line numbers at the left
  %numberstyle=\tiny\ttfamily, % style of the line numbers
  commentstyle=\color{eclipseBlue}, % style of comments
  keywordstyle=\bf\color{eclipsePurple}, % style of keywords
  stringstyle=\color{eclipseBlue}, % style of strings
}

\lstset{
language=modp,                 % the language of the code
}

